Coherent-Constructible Correspondence for Toric Fibrations

Let $\Sigma$ be a fan inside the lattice $\mathbb{Z}^n$, and $\mathcal{E}:\mathbb{Z}^n \rightarrow \operatorname{Pic}{S}$ be a map of abelian groups. We introduce the notion of a principal toric fibration $\mathcal{X}_{\Sigma, \mathcal{E}}$ over the base scheme $S$, relativizing the usual toric construction for $\Sigma$. We show that the category of ind-coherent sheaves on such a fibration is equivalent to the global section of the Kashiwara-Schapira stack twisted by a certain local system of categories with stalk $\operatorname{Ind}\operatorname{Coh} S$. It is a simultaneous generalization of the work of Harder-Katzarkov [HK19] and of Kuwagaki [Kuw20], and should be seen as a family-version of the coherent-constructible correspondence [FLTZ11].

==> sections/local-case.tex <==
\section{local case}
Consider the stacky fan data $(\hat\Sigma=\hat{\Sigma}(\hat\sigma),\beta)$
given by faces of a single rational strictly convex cone $\hat\sigma$ inside $L^\vee$.
In this case, $\Xc_{\hat\Sigma, \beta}\rightarrow Y$ is
(the stacky quotient of) an affine bundle.

Recall that the FLTZ skeleton is given by
\begin{equation}
\Lambda_{\hat\Sigma,\beta} = 
\bigcup_{\tau\in\hat\Sigma}\bigcup_{\chi \in M_{\tau,\beta}/M}(-\tau)\times (\tau^\perp + \chi) \subset T^*M_{T}.
\end{equation}

Let $\Uc=\coprod_{\alpha\in I} U_\alpha \rightarrow Y$ be a (finite) Zariski cover such that the image of $\Ec$ pulls-back to trivial line bundles.
% Denote by
% \[
% C(\Uc)=
% \cdots\rightarrow \Uc\times_Y\Uc\times_Y\Uc
% \rightarrow
% \Uc \times_Y \Uc
% \rightarrow
% \Uc
% \]
% the Cech nerve.
For any affine open $U_\alpha\rightarrow Y$. Consider the sheaves $\Phi_\alpha(\Ec)$ defined similarly but with
$\ind\coh(Y)$ replaced by $\ind\coh(U_\alpha)$.
\begin{lemma}
$\lim_{\alpha\in C(I)} \Phi_{\alpha}(\Ec) \simeq \Phi(\Ec)$.
\end{lemma}
\begin{proof}
It follows from Zariski descent of ind-coherent sheaves
and the fact that limits of sheaves are computed pointwise.
\end{proof}
Write $X_{\hat\Sigma(\hat\sigma), \beta}$ for the fiber of the fibration.

\begin{lemma}[{\cite[lemma 7.2]{kuwagaki20}}]
\[
X_{\hat\Sigma(\sigma), \beta}=[\spec\C[\hat\sigma^\vee \cap L^\vee]/G_\beta]\simeq[\spec\C[\sigma^\vee/\sigma^\perp\cap M_{\sigma,\beta}]/H_\beta].
\]
\end{lemma}

\begin{prop}
There is an equivalence functorial in $U_\alpha$ \[\Gamma(\ush_{\Lambda_{\hat\Sigma,\beta}}\otimes_{\C}\Phi_\alpha(\Ec))\simeq \ind\coh(\Xc_{\hat\Sigma,\beta}|_{U_\alpha}).\]
\end{prop}
\begin{proof}
Note that there are equivalences \cite[Corrolary 12.7]{kuwagaki20}
\[
\sh^w_{\Lambda_{\hat\Sigma,\beta}}(M_T)\simeq \coh(X_{\hat\Sigma,\beta}),
\]
\[
\sh^\diamond_{\Lambda_{\hat\Sigma,\beta}}(M_T) \simeq \ind\coh(X_{\hat\Sigma,\beta}),
\]
where the latter is obtained by taking ind-completion.

\end{proof}
